Identifying Domain Adjacent Instances for Semantic Parsers

When the semantics of a sentence are not representable in a semantic parser's output schema, parsing will inevitably fail. Detection of these instances is commonly treated as an out-of-domain classification problem. However, there is also a more subtle scenario in which the test data is drawn from the same domain. In addition to formalizing this problem of domain-adjacency, we present a comparison of various baselines that could be used to solve it. We also propose a new simple sentence representation that emphasizes words which are unexpected. This approach improves the performance of a downstream semantic parser run on in-domain and domain-adjacent instances.

==> direct_results_model.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
& Restaurants & Calendar & Social & Housing\\
\hline
\textsc{Autoencoder}&0.919&0.644&0.757&0.877\\
\textsc{Clustering}&0.883&0.569&0.797&0.734\\
\textsc{kNN}&0.914&0.685&0.805&0.923\\
\hline
\end{tabular}
}
\end{center}
\caption{AUC for domain-adjacent instance identification, using \textsc{CBOW} sentence representations.\todo{Why don't we use Surprise here?}}

\label{table:direct_eval_models}
\end{table}

==> downstream_results.tex <==
\begin{table*}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
& Basketball & Blocks & Calendar & Housing & Publications  & Recipes & Restaurants & Social \\
\hline
\textsc{Confidence} & -  & - & - & - & - & - & - & -  \\
\textsc{CBOW}       & 0.133 & 0.057 & 0.340 & 0.231 & 0.209 & 0.245 & 0.443 & 0.105     \\
\textsc{CNN}        & \textbf{0.174} & 0.108 & 0.406 & 0.238 & 0.295 & 0.329 & 0.488 & 0.138 \\
\textsc{LSTM}       & 0.132 & 0.096 & 0.404 & 0.228 & 0.294 & 0.297 & 0.441 & \textbf{0.150} \\
\textsc{Surprise}   & 0.122 & 0.090 & \textbf{0.423} & \textbf{0.280} & \textbf{0.308} & \textbf{0.377} & \textbf{0.535} & 0.131 \\
\hline
\end{tabular}
}
\end{center}
\caption{AUC for a semantic parser evaluated on a test set in which 20\% is domain adjacent.}
\label{table:downstream_eval}
\end{table*}

==> downstream_results_f1.tex <==
\begin{table*}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
& Basketball & Blocks & Calendar & Housing & Publications  & Recipes & Restaurants & Social \\
\hline
\textsc{NoFilter}	& 0.340	& 0.306	& 0.617	& 0.462	& 0.511	& 0.570	& 0.616	& 0.355 \\
\textsc{Oracle}	& 0.378	& 0.340	& 0.684	& 0.513	& 0.567	& 0.633	& 0.684	& 0.395 \\
\hline
\textsc{Autoencoder} & 0.319 & 0.258 & 0.530 & 0.364 & 0.416 & 0.524 & 0.484 & 0.340 \\
\hline
\textsc{Confidence}	& \textbf{0.347} & 0.306 & 0.629	& 0.478	& 0.512	& \textbf{0.567}	& 0.639	& 0.359 \\
\hline
\textsc{CBOW}	& 0.325	& 0.283	& 0.597	& 0.451	& 0.541	& 0.559	& 0.641	& 0.348 \\
\textsc{CNN}	& 0.347	& 0.301	& 0.582	& 0.468	& 0.515	& 0.566	& 0.583	& \textbf{ 0.360} \\
\textsc{LSTM}	& 0.336	& 0.303 & 0.565 & 0.432 & 0.485 & 0.558 & 	0.599 & 0.349 \\
\textsc{Surprise} & 0.342 & \textbf{0.310} & \textbf{0.633} & \textbf{0.481} & \textbf{0.560} & 0.552 & \textbf{0.662} & 0.343 \\
\hline
\end{tabular}
}
\end{center}
\caption{F1 for a semantic parser evaluated on a test set in which 20\% is domain adjacent.}
\label{table:downstream_eval}
\vspace{-.25cm}
\end{table*}
